Resolution Enhancement of Scanning Electron Micrographs using Artificial Intelligence

Scanning Electron Microscopy (SEM) is pivotal in revealing intricate micro- and nanoscale features across various research fields. However, obtaining high-resolution SEM images presents challenges, including prolonged scanning durations and potential sample degradation due to extended electron beam exposure. This paper addresses these challenges by training and applying a deep learning based super-resolution algorithm. We show that the chosen algorithm is capable of increasing the resolution by a factor of 4, thereby reducing the initial imaging time by a factor of 16. We benchmark our method in terms of visual similarity and similarity metrics on two different materials, a dual-phase steel and a case-hardening steel, improving over standard interpolation methods. Additionally, we introduce an experimental pipeline for the study of rare events in scanning electron micrographs, without losing high-resolution information.

==> notes.tex <==
de Haan et al have used generative adversarial networks in order to enhance the resolution in scanning electron microscopy
images. The specific use case, that they argue is that for certain materials (e.g. biological samples) long exposure to
high energy electrons can be harmful. Scanning with a lower resolution and then using super resolution would thereby
enable the scanning of such materials. Furthermore, they argue that spherical aberrations and noise can be corrected using
super resolution algorithms. \\
Our approach sees a different application, where the goal is not necessarily the sensitive material, but experiments where
similar surfaces are scanned multiple times, and a stack of high resolution images is already available. This stack together
with a pretrained and then finetuned texture transformer network, can produce realistic high resolution images, that can then
be used for high resolution rescanning of points of interest. Points of interest can be found by finetuning YOLO or a similar
algorithm to points of interest, e.g. nano indents. \\
One more difference is the dataset generation. While the dataset generation in this paper is similar to the paper by microsoft
in the eye of the researcher, the additional complexity is unnecessary. As a scanning electron scans a material and the corresponding
low resolution image is just a subset of the high resolution image, given all other parameter being equal. Using this information
any lab can fine tune their texture transformer quickly, by just recording a few images, subsampling them, and then fine tuning
or completely training TTSR from anew.\\
